Flexible Coinduction in Agda

Theorem provers are tools that help users to write machine readable proofs. Some of this tools are also interactive. The need of such softwares is increasing since they provide proofs that are more certified than the hand written ones. Agda is based on type theory and on the propositions-as-types correspondence and has a Haskell-like syntax. This means that a proof of a statement is turned into a function. Inference systems are a way of defining inductive and coinductive predicates and induction and coinduction principles are provided to help proving their correctness with respect to a given specification in terms of soundness and completeness. Generalized inference systems deal with predicates whose inductive and coinductive interpretations do not provide the expected set of judgments. In this case inference systems are enriched by corules that are rules that can be applied at infinite depth in a proof tree. Induction and coinduction principles cannot be used in case of generalized inference systems and the bounded coinduction one has been proposed. We first present how Agda supports inductive and coinductive types highlighting the fact that data structures and predicates are defined using the same constructs. Then we move to the main topic of this thesis, which is investigating how generalized inference systems can be implemented and how their correctness can be proved.

==> codes/latex/mystream_memberOf.tex <==
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}memberOf\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSymbol{\}(}\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{)(}\AgdaBound{l}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{MyStream}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{mem{-}b}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaField{MyStream.hd}\AgdaSpace{}%
\AgdaBound{l}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{memberOf}}\AgdaSpace{}%
\AgdaBound{l}\<%
\\
%
\>[2]\AgdaInductiveConstructor{mem{-}i}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{memberOf}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaField{MyStream.tl}\AgdaSpace{}%
\AgdaBound{l}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[40]\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{memberOf}}\AgdaSpace{}%
\AgdaBound{l}\<%
\\
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{mem{-}eq}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{MyStream}\AgdaSpace{}%
\AgdaDatatype{Nat}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{i}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Nat}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{get}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{i}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{memberOf}}\AgdaSpace{}%
\AgdaBound{s}\<%
\\
\>[0]\AgdaFunction{mem{-}eq}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaInductiveConstructor{zero}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{mem{-}b}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{mem{-}eq}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{i}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{mem{-}i}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{mem{-}eq}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaField{MyStream.tl}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{i}\AgdaSymbol{)}\<%
\\
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{mem{-}eq2}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSymbol{\}\{}\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{\}\{}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{MyStream}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{memberOf}}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{∃}\AgdaSpace{}%
\AgdaDatatype{Nat}\AgdaSpace{}%
\AgdaSymbol{(λ}\AgdaSpace{}%
\AgdaBound{i}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{get}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{i}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{mem{-}eq2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{mem{-}b}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{<}}\AgdaSpace{}%
\AgdaInductiveConstructor{zero}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaFunction{sym}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{>}}\<%
\\
\>[0]\AgdaFunction{mem{-}eq2}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{s}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{mem{-}i}\AgdaSpace{}%
\AgdaBound{p}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{<}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{witness}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{mem{-}eq2}\AgdaSpace{}%
\AgdaBound{p}\AgdaSymbol{)))}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaFunction{proof}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{mem{-}eq2}\AgdaSpace{}%
\AgdaBound{p}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{>}}\<%
\end{code}



==> sections/agda-approaches.tex <==
\subsection{Comments}
We presented two different implementations of colists. The standard library provides a code that deals with infinite object taking advantage from the concept of approximation. Two additional data types are involved, Thunk and Size. The first is the type of suspended computations and it must be used to simulate laziness while the second specifies the approximation and can be $\infty$. It is also necessary to let the termination checker know that the size of the data decreases when the computation is forced.
Those concepts can make the overall data types a little bit obscure because they add variables that must be correctly understood when writing a code. On the other hand the proofs are simple and follow the scheme adopted for finite lists; also the syntax is similar. The do not need complex passages because they are based on how the lists are built. There is no need to use different techniques (\textit{pattern, copattern matching}) when dealing with inductive and coinductive predicates.
\\\\
Our approach aims at implementing colists in a consistent way with respect to how coinduction is managed in Agda. The resulting type is intuitive due to the coinductive record adoption. The same can be said for coinductive predicates. In this case different techniques must be used according to the kind of the predicate. 
The main challenges are the auxiliary equalities that must be written since the proofs are based on how the lists are observed; thus the variables inside the types must be related to those inside the proofs.
This fact becomes more evident when predicates that are not unary are considered (e.b. binary relations).
\\\\
In the next chapter we are going to adopt again both strategies.

==> sections/agda-equality.tex <==
\section{Agda Equality Properties}\label{sect:eqproperties}

This is the module containing the implementations of the equality properties which is not present inside the builtin library. They are defined as functions that take as input equality proofs. Notice that  \textit{refl} is written as an argument in function definitions because if for example the proof asks for an argument of type $x \equiv y$, there is only one allowed constructor. In order to be sure of this fact one could replace the direct constructor with a variable, e.g. $eq$, of that type and then pattern matching on it interactively. The result that would be obtained is the one above. This and other syntactical elements are going to be better explained next. It must be clear that the outputs are not boolean values but actually equality proofs. Let $eq$ be the proof that $x$ is equal to $y$ where $x, y$ have type $A$ leading to a term of type $x \equiv y$, then \textit{sym eq} returns a term of type $y \equiv x$. No additional input elements must be provided to that function.

\begin{center}
\input{codes/latex/EqProperties}
\end{center}



==> sections/inference_systems.tex <==
\chapter{Inference Systems}

==> sections/temporal-operators-agda.tex <==
\section{Temporal Operators In Agda}
\label{temp-op}

In this section we propose the implementations in Agda of the different operators involving generic unary predicates on possibly infinite data structures. Then we provide the soundness and completeness proofs. The codes are based both on the standard library module and our approach for colists. 
The first two operators recall what was presented in the previous chapter since they generalize the predicates that were analyzed.



\subsection{Always}



==> sections/temporal-operators-is.tex <==
\section{\EZ{Inference systems}}
\label{temp-op-is}

\EZ{In this section we show how to define the four parametric predicates by inference systems.}






